BlockFLow: An Accountable and Privacy-Preserving Solution for Federated Learning

Federated learning enables the development of a machine learning model among collaborating agents without requiring them to share their underlying data. However, malicious agents who train on random data, or worse, on datasets with the result classes inverted, can weaken the combined model. BlockFLow is an accountable federated learning system that is fully decentralized and privacy-preserving. Its primary goal is to reward agents proportional to the quality of their contribution while protecting the privacy of the underlying datasets and being resilient to malicious adversaries. Specifically, BlockFLow incorporates differential privacy, introduces a novel auditing mechanism for model contribution, and uses Ethereum smart contracts to incentivize good behavior. Unlike existing auditing and accountability methods for federated learning systems, our system does not require a centralized test dataset, sharing of datasets between the agents, or one or more trusted auditors; it is fully decentralized and resilient up to a 50% collusion attack in a malicious trust model. When run on the public Ethereum blockchain, BlockFLow uses the results from the audit to reward parties with cryptocurrency based on the quality of their contribution. We evaluated BlockFLow on two datasets that offer classification tasks solvable via logistic regression models. Our results show that the resultant auditing scores reflect the quality of the honest agents' datasets. Moreover, the scores from dishonest agents are statistically lower than those from the honest agents. These results, along with the reasonable blockchain costs, demonstrate the effectiveness of BlockFLow as an accountable federated learning system.

==> junk.tex <==

Given the distributed nature of federated learning, blockchains provide an ideal environment to manage a federated learning experiment. A smart contracts can audit each client's submission and award virtual currency to those who make the most meaningful contributions. It can also expel clients who fail to follow the protocol. Clients need not trust a centralized authority to ensure that their models were evaluated fairly and that they received the correct payment; instead; they must only trust the verifiable and freely accessible smart contract bytecode.

BlockFLow is a .....

BlockFLow requires all parties to post a bond to the Ethereum blockchain smart contract upon enrolling in the experiment. A party forfeits this bond if one fails to follow the protocol. For each federated learning round, all parties submit both their models and evaluations on all other parties' models to an Ethereum blockchain smart contract. The Smart Contract then computes overall scores for each party. Since the scoring algorithm penalizes parites who improperly evaluate others' models, the only nash equilibrium with a sufficiently large bond would be to be honest. These scores indicate which clients, if any, might have submitted a malicious model. In addition, the smart contract pays the clients (via cryptocurrency) pro-rata according to their scores. The scoring algorithm, and the Ethereum blockchain network, are resilient up to 51\% attack in a malicious trust model. Thus, BlockFLow can be used in any federated learning environment.




\subsection{Decentralized Federated Learning}
\label{sec:background:decentralized_federated_learning}
Let there be $N$ clients who want to train a collaborative machine learning model $W_{fed}$ without exposing their datasets to each other. With decentralized federated learning, all clients $i \in N$ train a local model $w_i$ with their own data. At an agreed upon deadline, clients share their models with each other, and average everyone's model together. This process repeats for a pre-defined number of rounds.

% \begin{algorithm}
% \SetAlgoLined
%     \begin{algorithmic}[]
%         \FORALLP{$\text{clients } i \in N$}
%             \STATE{$w^1_i \gets \text{random initialization}$}
%             \FOR{$r \gets 1 \text{ to } R$}
%                 \STATE $w^r_i \gets \text{train}(r, w^r_i)$ \COMMENT{See Algorithm \ref{alg:training_procedure}}
%                 \FORALLP{$\text{clients } k \in n$}
%                     \STATE{$\text{send model } w_i \text{ to client } k$} \\
%                     \STATE{$w_k \gets \text{ receive model from client } k$}
%                 \ENDFOR\\
%                 \STATE{$w_i \gets \frac{1}{n}\sum_{k=1}^{n} w_{k} $} \COMMENT{all clients should now have identical $w_i$}
%             \ENDFOR\\
%         \ENDFOR\\
%     \end{algorithmic}
%     \caption{Procedure Decentralized Federated Learning}
%     \label{alg:federated_learning}
% \end{algorithm}

% \begin{algorithm}
% \SetAlgoLined
%     \begin{algorithmic}[]
%         \REPEAT
%             \STATE $w^r_i \gets w^r_i - \eta \nabla g(w^r_i)$
%         \UNTIL{deadline for round $r$}
%         \RETURN $w^r_i$
%     \end{algorithmic}
%     \caption{Training Procedure for round $r$, client $i$, weights $w^r_i$}
%     \label{alg:training_procedure}
% \end{algorithm}




The blockchain is maintained by independent nodes, known as ``miners''. Public-private key cryptography secures the accounts for miners and other blockchain users. To append to the ledger, users must sign transactions with their private keys, include a fee (in virtual currency), and broadcast it to the miners. A transaction could denote the transfer of currency or the execution of smart contract. A miner combines this transaction with others into a ``block''.  The first miner to solve an NP-hard problem is rewarded with new virtual currency and all the fees from the transactions in the block. Other miners will only accept the block upon verification the NP-hard proof. The longest ``chain`` of blocks is considered to be the correct state of the blockchain. This process, called ``mining,'' ensures that all nodes are in-sync and reflect the same state of the network, even without a centralized authority.



For example, consider a scenario where many health care providers want to develop model. With federated learning, each provider would train a model on their data and send this model, rather than the data, to a centralized server. This centralized server would then average such models and send the averaged model back to the participants. Participants then train on their dataset, starting from the shared model. This process repeats until convergence. Federated machine learning generally improves model accuracy relative to each client's initial, individual model \cite{something}.







The formal client procedure is detailed in algorithm \ref{alg:client_procedure}.

\begin{algorithm}
\SetAlgoLined
    \begin{algorithmic}[]
        \REQUIRE {$\text{client } i \in N$}
        \REQUIRE{$\text{evaluate}(x) \in [0, 1] \quad \forall x$} \COMMENT{evaluate must be a function where $\text{evaluate}(x) > \text{evaluate}(x') \iff$  model $x$ is better than model $x'$; $\text{evaluate}(x) = 1.0 \iff$  model $x$ is perfect; and $\text{evaluate}(x) > 0.0 \implies$  model $x$ is valid} \\
        \STATE{}
        \STATE{$\text{client } i \text{ posts bond } b \text{ to BlockFLow smart contract }$}
        \STATE{}
        \STATE{In a background process, do:}
        \REPEAT
            \FORALL{$\text{clients } k \in N$}
                \IF{client $k$ requests $w_k'^r$ for client $k'$ and $w_k'^r$ is valid}
                    \STATE{encrypt $w_k'^r$ and share with client $k$}
                \ENDIF
            \ENDFOR
        \UNTIL{$\text{forever, in background}$}
        \STATE{}
        \STATE{In the main process, do:}
        \FOR{$\text{round } r \gets 1 \text{ to } R$}
            \STATE{$N \gets N \setminus \text{ \{expelled clients\}}$} \COMMENT{Clients who failed to follow smart contract procedure in $r-1$ are expelled}
            \REPEAT
                \STATE $w^r_i \gets w^r_i - \eta \nabla g(w^r_i)$
            \UNTIL{deadline for round $r$}
            \STATE $w^r_i \gets w^r_i+Lap(0, \frac{2}{d_i\alpha\epsilon})$
            \STATE{$a_i^r \gets $ encrypt and upload model $w_i^r$ to IPFS and record the address}
            \STATE{record model IPFS address $a_i^r$ in BlockFLow smart contract}
            \FORALL{$\text{clients } k \in n$}
                \STATE{$a_k^r \gets$ get client $k$ model's IPFS address from smart contract}
                \STATE{$w_k^r \gets \text{load and validate model } a_k^r$}
                \IF{$w_k^r \text{ is valid}$}
                    \STATE{report $w_k^r$ as valid in BlockFLow smart contract}
                \ENDIF
            \ENDFOR
            \STATE{wait for data retrieval deadline}
            \FORALL{$\text{clients } k \in N$}
                \STATE{$v^r_k \gets $ count number of models client $k$ marked as valid}
                \STATE{$z^r_k \gets $ count number of clients who marked client $k$'s model as valid}
                \IF{$v^r_k \le \frac{N}{2} \text{ or } z^r_k \le \frac{N}{2}$}
                    \STATE{expel client $k$}
                    \STATE{$N \gets N \setminus k$}
                \ELSE
                    \IF{agent $i$ does not have valid model $w_k^r$}
                        \FORALL{$\text{clients }k' \in N$}
                            \STATE{$w_k^r \gets $ request and retrieve model $k$ from client $k'$} \COMMENT{Guaranteed to work for some $k' \in N$; see threat analysis in section \ref{sec:threat_analysis:ipfs_data_sharing} }
                        \ENDFOR
                    \ENDIF
                    \STATE{$s^r_{i, k} \gets \text{evaluate}_i(w_k^r)$}
                    \STATE{$b^r_{i, k} \gets \text{random encryption key}$}
                    \STATE{$s'^r_{i, k} \gets \text{encrypt}_{b^r_{i, k}}(w_k^r)$}
                    \STATE{report encrypted score $s'^r_{i, k}$ for client $k$ to smart contract}
                \ENDIF
            \ENDFOR
            \STATE{Wait for before encrypted score submission deadline}
            \FORALL{$\text{clients } k \in N$}
                \STATE{provide decryption key $b^r_{i, k}$ to provably reveal score $s^r_{i, k})$ to smart contract}
            \ENDFOR
            \STATE{Wait for score decryption submission deadline}
            \STATE{$p' \gets \text{ get scores from smart contract}$} \COMMENT{See Algorithm \ref{alg:scoring_procedure}}
            \STATE{$w_i^{r+1} \gets \frac{\sum_{k=1}^{n}(w^r_{k}*p'_k)}{n * \sum_{k=1}^{n}(p'_k)} $} \COMMENT{all clients should now have identical $w_i^{r+1}$}
        \ENDFOR\\
    \end{algorithmic}
    \caption{BlockFLow Client Procedure}
    \label{alg:client_procedure}
\end{algorithm}


to be appropriate 

homomorphic encryption \cite{aono2017privacy,hall2011secure}, and differential privacy \cite{dwork2010differential} are the most commonly used techniques to guarantee security and privacy of machine learning algorithms in a federated learning environment. 

Differential privacy \cite{dwork2006calibrating} provides the necessary protection against these types of inference attacks. This is done by adding random noise to the input data or model parameters. The above mentioned combination of MPC and differential privacy provides the necessary guarantees under a semi-honest setting where agents follow a specified protocol.

Numerous approaches have been proposed to enhance privacy and security in a federated learning environment. \cite{mcmahan2017learning} and \cite{dwork2010differential} applied differential privacy to provide the necessary privacy guarantees whereas \cite{bonawitz2017practical} proposed a secure aggregation protocol for privacy-preserving machine learning in a federated environment.

homomorphic encryption \cite{aono2017privacy,hall2011secure}, and differential privacy \cite{dwork2010differential} are the most commonly used techniques to guarantee security and privacy of machine learning algorithms in a federated learning environment. 



\cite{benhamouda2019supporting} propose a privacy-preserving platform using MPC on Hyperledger Fabric \cite{androulaki2018hyperledger}. Their work is useful for applications which need exact computation and isn't useful for learning models from data. 






discussed in \ref{sec:threat_analysis:scoring} -- specifically, those identified i where multiple agents collude in the evaluation. We do not view the private sharing of datasets as collusion, as doing so would invalidate the differential the colluding agents' privacy guarantees. Differential privacy is robust up to n-1 colluding agents \cite{goryczka2013secure,bindschaedler2017achieving}. From the prospective of the honest agents, this scenario is no different where some agents have significantly larger datasets than others. This case was already analyzed in Experiment 2. Hence, we discuss collusion attacks that do not involve the sharing of training datasets -- specifically, the fabrication of evaluation scores. Note that collusion is NOT game-theory optimal, for two reasons: first, one's evaluation score will be further from the median, as determined by the honest agents, and secondly, game theory strategies to achieve a higher payoff with collusion, such as those that depend upon the folk theorem \cite{dutta1995folk, fudenberg2009folk} do not apply in finitely-repeating games, such as federated learning, where the number of rounds is upper bounded. Nonetheless, we examined the worst-case scenario where the colluding agents report a score of 1.0 for each-others' models and 0.0 for the honest agents' models. We re-evaluated the models from experiment 1 after randomly selecting a subset of the agents to collude in this manner. We present in figure TODO how the scoring algorithm, by using median instead of mean, is robust against this type of collusion. 


